FPIA: Field-Programmable Ising Arrays with In-Memory Computing

Ising Machine is a promising computing approach for solving combinatorial optimization problems. It is naturally suited for energy-saving and compact in-memory computing implementations with emerging memories. A na\"ive in-memory computing implementation of a quadratic Ising Machine requires an array of coupling weights that grows quadratically with problem size. However, the resources in such an approach are used inefficiently due to sparsity in practical optimization problems. We first show that this issue can be addressed by partitioning a coupling array into smaller sub-arrays. This technique, however, requires interconnecting subarrays; hence, we developed in-memory computing architecture for quadratic Ising Machines inspired by island-type field programmable gate arrays, which is the main contribution of our paper. We adapt open-source tools to optimize problem embedding and model routing overhead. Modeling results of benchmark problems for the developed architecture show up to 60x area improvement and faster operation than the baseline approach. Finally, we discuss algorithm/circuit co-design techniques for further improvements.

==> fig/FPIA_schematic/FPIA_schematic_floorplan.tikz.tex <==
\begin{tikzpicture}[
    node distance=0.5,
    tile/.style={minimum width=30.0,minimum height=30.0, draw, rectangle, fill=white}
    ]
    \node[tile] (S00) {S};
    \node[tile, right=of S00] (C10) {C};
    \node[tile, below=of S00] (C01) {C};
    \node[tile, below=of C10, rectangle] (IMC11) {IMC};
    \node[tile, right=of C10, rectangle] (S20) {S};
    \node[tile, right=of S20, rectangle] (C30) {C};
    \node[tile, below=of S20, rectangle] (C21) {C};
    \node[tile, below=of C30, rectangle] (IMC31) {IMC};
    \node[tile, below=of C01, rectangle] (S02) {S};
    \node[tile, right=of S02, rectangle] (C12) {C};
    \node[tile, below=of S02, rectangle] (C03) {C};
    \node[tile, below=of C12, rectangle] (IMC13) {IMC};
    \node[tile, right=of C12, rectangle] (S22) {S};
    \node[tile, right=of S22, rectangle] (C32) {C};
    \node[tile, below=of S22, rectangle] (C23) {C};
    \node[tile, below=of C32, rectangle] (IMC33) {IMC};
    
    \node[tile, right=of C30] (S40) {S};
    \node[tile, right=of IMC31] (C41) {C};
    \node[tile, right=of C32] (S42) {S};
    \node[tile, right=of IMC33] (C43) {C};
    \node[tile, below=of C03] (S04) {S};
    \node[tile, below=of IMC13] (C14) {C};
    \node[tile, below=of C23] (S24) {S};
    \node[tile, below=of IMC33] (C34) {C};
    \node[tile, below=of C43] (S44) {S};
    
    \draw ($(S00.north west)+(-0.0,1.5)$)  rectangle ($(S40.north east)+(0.0,0.5)$) node [pos=0.5] () { \Large Programming};
    \draw ($(S00.north west)+(-1.5, 0.0)$) rectangle ($(S04.south west)+(-0.5, 0.0)$) node [rotate=90, pos=0.5] () { \Large Programming};
    \begin{scope}[on background layer]
        \draw (S00.30) -- (S40.150);
        \draw (S00.0) -- (S40.180);
        \draw (S00.-30) -- (S40.-150);

        \draw (S02.30) -- (S42.150);
        \draw (S02.0) -- (S42.180);
        \draw (S02.-30) -- (S42.-150);

        \draw (S04.30) -- (S44.150);
        \draw (S04.0) -- (S44.180);
        \draw (S04.-30) -- (S44.-150);

        \draw (S00.-60) -- (S04.60);
        \draw (S00.-90) -- (S04.90);
        \draw (S00.-120) -- (S04.120);

        \draw (S20.-60) -- (S24.60);
        \draw (S20.-90) -- (S24.90);
        \draw (S20.-120) -- (S24.120);

        \draw (S40.-60) -- (S44.60);
        \draw (S40.-90) -- (S44.90);
        \draw (S40.-120) -- (S44.120);

        \draw [ultra thick] (C01.0) -- (C41.180);
        \draw [ultra thick] (C03.0) -- (C43.180);
        \draw [ultra thick] (C10.-90) -- (C14.90);
        \draw [ultra thick] (C30.-90) -- (C34.90);

        
    \end{scope}
\end{tikzpicture}

==> fig/FPIA_schematic/IMC_tile_schematic+floorplan.tikz.tex <==
\begin{tikzpicture}[
        % every node/.style={draw,outer sep=0pt,thick},
        neuron/.style  = {draw,thick,fill=blue!20, regular polygon, regular polygon sides=3, shape border rotate=-90},
        xp/.style = {draw,thick,circle, fill=green!40},
        sh/.style = {draw,thick,rectangle, anchor=center, fill=blue!40},
        scale=0.9
    ]
    \draw (0,0) node [xp] (xp11) {};
    \draw (1,0) node [xp] (xp12) {};
    \draw (2,0) node [xp] (xp13) {};
    \draw (3,0) node [xp] (xp14) {};
    \draw (0,-1) node [xp] (xp21) {};
    \draw (1,-1) node [xp] (xp22) {};
    \draw (2,-1) node [xp] (xp23) {};
    \draw (3,-1) node [xp] (xp24) {};
    \draw (0,-2) node [xp] (xp31) {};
    \draw (1,-2) node [xp] (xp32) {};
    \draw (2,-2) node [xp] (xp33) {};
    \draw (3,-2) node [xp] (xp34) {};
    \draw (0,-3) node [xp] (xp41) {};
    \draw (1,-3) node [xp] (xp42) {};
    \draw (2,-3) node [xp] (xp43) {};
    \draw (3,-3) node [xp] (xp44) {};
    \draw (4,0) node [xp] (xpb1) {};
    \draw (4,-1) node [xp] (xpb2) {};
    \draw (4,-2) node [xp] (xpb3) {};
    \draw (4,-3) node [xp] (xpb4) {};

    \draw [thick] ($(xp11.north west)+(-0.2,0.2)$) rectangle ($(xpb4.south east)+(+0.2,-0.2)$);
    \draw ($(xp13.north)+(0.0,0.15)$) node [anchor=south] () {$I \cdot O \cdot A_{cell}$};

    \coordinate[] (tmp_nw) at ($(xpb1.north east)+(0.7,0.1)$);
    \coordinate[] (tmp_se) at ($(xpb4.south east)+(1.3,-0.1)$);
    \node [fit=(tmp_nw) (tmp_se), thick, draw, fill=green!5] (bl_overhead) {};
    \draw (bl_overhead) node [] () {\rotatebox[origin=c]{90}{Output Overhead}};
    \coordinate[] (tmp_nw) at ($(xpb1.north east)+(2.2,0.1)$);
    \coordinate[] (tmp_se) at ($(xpb4.south east)+(2.8,-0.1)$);
    \node [fit=(tmp_nw) (tmp_se), thick, draw, fill=red!10] (neurons) {};
    \draw (neurons) node [] () {\rotatebox[origin=c]{90}{Spins \& Annealing}};
    \draw ($(xpb1.north east)+(1.8,0.15)$) node [anchor=south] () {$O \cdot (A_{bl} + A_{sense})$};

    \begin{scope}[on background layer]
        \draw (xp11.center) -- (xpb1.east) -- +(0.6,0.0);
        \draw (xp21.center) -- (xpb2.east) -- +(0.6,0.0);
        \draw (xp31.center) -- (xpb3.east) -- +(0.6,0.0);
        \draw (xp41.center) -- (xpb4.east) -- +(0.6,0.0);
        \draw [blue] (xp11.center) -- (xp41.south) -- +(0.0,-0.6);
        \draw [blue] (xp12.center) -- (xp42.south) -- +(0.0,-0.6);
        \draw [blue] (xp13.center) -- (xp43.south) -- +(0.0,-0.6);
        \draw [blue] (xp14.center) -- (xp44.south) -- +(0.0,-0.6);
        \draw [blue] (xpb1.center) -- (xpb4.south) -- +(0.0,-0.6);
    \end{scope}


    \coordinate[] (tmp_nw) at ($(xp41.south west)+(-0.1,-0.8)$);
    \coordinate[] (tmp_se) at ($(xpb4.south east)+(0.1,-1.4)$);
    \node [fit=(tmp_nw) (tmp_se), draw, thick, fill=green!5] (wl_overhead) {};
    \draw (wl_overhead) node [] () {Input Overhead};
    % \draw [thick,fill=green!5] ($(xp41.south west)+(-0.2,-0.6)$) rectangle node [] (wl_overhead) {Input Overhead} ($(xpb4.south east)+(0.2,-1.6)$);
    \draw ($(wl_overhead.east)+(0.2,0)$) node [anchor=west] () {$I \cdot A_{wl}$};

    % \draw ($(neurons.east)+(1.8,0.0)$) node [draw, thick, rectangle, fill=blue!20, anchor=west] (outpins) { \rotatebox{90}{Output Pins} };
    \draw ($(wl_overhead.-150)+(0.0,-0.9)$) node [draw, thick, rectangle, fill=blue!20, anchor=north] (inpins) {Input Pins};
    \draw ($(inpins)+(6.0,0.0)$) node [draw, thick, rectangle, fill=blue!20] (outpins) {Output Pins};

    \draw [ultra thick, -stealth] (bl_overhead.east) -- (neurons.west);

    \draw[-stealth,blue,ultra thick] (inpins) -- (inpins |- wl_overhead.south);
    \draw[-stealth,blue,ultra thick] (neurons.east) -- +(1.0,0.0) node [] (ohub) {}  -- +(1.0, -3.7) -| (wl_overhead.-30);
    \draw[-stealth,blue,ultra thick] (ohub) -- (ohub |- outpins.north);

    \draw [thick] ($(xp11.north west)+(-0.5,+0.75)$) rectangle ($(inpins.south -| outpins.east)+(0.0,-0.0)$);

    % \draw (outpins.east) node [single arrow, fill=blue!50, single arrow head extend=4.0, minimum width=2cm, anchor=west] () {\Large \textbf{To}};
    \draw (outpins.south) node [single arrow, fill=blue!50, single arrow head extend=4.0, minimum width=2cm, rotate=-90, anchor=west] () {\rotatebox[origin=c]{180}{\Large \textbf{To}}};
    \draw (inpins.south) node [single arrow, fill=blue!50, single arrow head extend=4.0, minimum width=2cm, rotate=90, anchor=east] () {\Large \textbf{From}};
    \draw [line width=0.25cm, -stealth] (0.5,-3.6) |- (4.8,-0.5);
    
    
    
\end{tikzpicture}

==> fig/IMC_tile_floorplan.tikz.tex <==
\begin{tikzpicture}[every node/.style={draw,outer sep=0pt,thick}]
    \node[draw, minimum size=2cm, regular polygon, 
        regular polygon sides=4, 
        label=side 2:$h_{cell}*O$, label=side 3:$w_{cell}*I$] (PXB) {Primary IMC crossbar};
    \node[draw, right=of PXB, minimum height=2cm, minimum width=1cm, rectangle, label=below:$w_{rblsw}$] (RBLSW) {Output periphery overhead};
    \node[draw, right=of RBLSW, minimum height=2cm, minimum width=1cm, rectangle, label=below:$w_{neuron}$] (sense) {Neurons};
    \node[draw, right=of sense, circle] (O) {Tile output pins};
    \node[draw, below=of O, circle] (I) {Tile input pins};
    \node[draw, rectangle, below=of PXB, label=left:$h_{rwlsw}$] (RWLSW) {Input periphery overhead};
    \draw [-latex] (PXB) -- (RBLSW);
    \draw [-latex] (RBLSW) -- (sense);
    \draw [-latex] (sense) -- (O);
    \draw [-latex] (sense) |- (RWLSW.north east);
    \draw [-latex] (I.west) |- (RWLSW.south east);
    \draw [-latex] (RWLSW) -- (PXB);
    \draw [thick, label=above:"IMC tile"] ($(PXB.north west)+(-1.6,0.6)$)  rectangle ($(I.south east)+(0.5,-0.6)$);
\end{tikzpicture}

==> fig/SRAM_coupler.tikz.tex <==

\begin{circuitikz}[american]
  \draw (0,0) node [draw,twoport,minimum height=1.5cm,minimum width=2cm] (mem00) {\Large 6T}; 
  \node [draw,nmos,anchor=G,right=0.3cm of mem00.east] (M00r0) {$1W$};
  \node [draw,nmos,below=0.3cm of M00r0] (M00r1) {$1W$};
  \draw (M00r0.S) to [short] (M00r1.D);
  \draw (M00r1.S) node [ground] () {};
  \draw (mem00.east) to [short] (M00r0.G);
  \draw (M00r1.G) to [short] ++(0.0cm, +0.5cm) to [short] ++(-2.5cm,0.0cm) node (RWL_in) {} node [above] () {RWL};
  \draw (M00r0.D) to [short] ++(+0.8cm, 0.0cm) to [short] ++(0.0cm, -10.0cm) node (RBL+_out) {} node [left] () {RBL+};
  \draw (0,0) node [draw,twoport,minimum height=1.5cm,minimum width=2cm,right=3cm of mem00] (mem01) {\Large 6T}; 
  \node [draw,nmos,anchor=G,right=0.3cm of mem01.east] (M01r0) {$1W$};
  \node [draw,nmos,below=0.3cm of M01r0] (M01r1) {$1W$};
  \draw (M01r0.S) to [short] (M01r1.D);
  \draw (M01r1.S) node [ground] () {};
  \draw (mem01.east) to [short] (M01r0.G);
  \draw (M01r1.G) |- (RWL_in);
  \draw (M01r0.D) to [short] ++(+0.8cm, 0.0cm) to [short] ++(0.0cm, -10.0cm) node (RBL-_out) {} node [left] () {RBL-};
  \draw (0,0) node [draw,twoport,minimum height=1.5cm,minimum width=2cm,below=3cm of mem00] (mem10) {\Large 6T}; 
  \node [draw,nmos,anchor=G,right=0.3cm of mem10.east] (M10r0) {$2W$};
  \node [draw,nmos,below=0.3cm of M10r0] (M10r1) {$2W$};
  \draw (M10r0.S) to [short] (M10r1.D);
  \draw (M10r1.S) node [ground] () {};
  \draw (mem10.east) to [short] (M10r0.G);
  \draw (M10r1.G) |- (RWL_in);
  \draw (M10r0.D) -| (RBL+_out);
  \draw (0,0) node [draw,twoport,minimum height=1.5cm,minimum width=2cm,right=3cm of mem10] (mem11) {\Large 6T}; 
  \node [draw,nmos,anchor=G,right=0.3cm of mem11.east] (M11r0) {$2W$};
  \node [draw,nmos,below=0.3cm of M11r0] (M11r1) {$2W$};
  \draw (M11r0.S) to [short] (M11r1.D);
  \draw (M11r1.S) node [ground] () {};
  \draw (mem11.east) to [short] (M11r0.G);
  \draw (M11r1.G) |- (RWL_in);
  \draw (M11r0.D) -| (RBL-_out);
\end{circuitikz}


==> fig/isaac_like_arch/isaac_like_arch.tikz.tex <==
\begin{tikzpicture}[
        neuron/.style  = {draw,thick,fill=blue!20, regular polygon, regular polygon sides=3, shape border rotate=-90},
        xp/.style = {draw,thick,circle, fill=green!40},
        sh/.style = {draw,thick,rectangle, anchor=center, fill=blue!40},
        scale=1.0
    ]
    \begin{scope}[shift={(0,0)}]
        \begin{scope}[shift={(0,0)}]
            \draw (0,0) node [xp] (xp11) {};
            \draw (1,0) node [xp] (xp12) {};
            \draw (2,0) node [xp] (xp13) {};
            \draw (3,0) node [xp] (xp14) {};
            \draw (0,-1) node [xp] (xp21) {};
            \draw (1,-1) node [xp] (xp22) {};
            \draw (2,-1) node [xp] (xp23) {};
            \draw (3,-1) node [xp] (xp24) {};
            \draw (0,-2) node [xp] (xp31) {};
            \draw (1,-2) node [xp] (xp32) {};
            \draw (2,-2) node [xp] (xp33) {};
            \draw (3,-2) node [xp] (xp34) {};
            \draw (0,-3) node [xp] (xp41) {};
            \draw (1,-3) node [xp] (xp42) {};
            \draw (2,-3) node [xp] (xp43) {};
            \draw (3,-3) node [xp] (xp44) {};
            \draw (4,0) node [xp] (xpb1) {};
            \draw (4,-1) node [xp] (xpb2) {};
            \draw (4,-2) node [xp] (xpb3) {};
            \draw (4,-3) node [xp] (xpb4) {};
        
            \draw (5.3,0) node [sh] (sh1) {S\&H};
            \draw (5.3,-1) node [sh] (sh2) {S\&H};
            \draw (5.3,-2) node [sh] (sh3) {S\&H};
            \draw (5.3,-3) node [sh] (sh4) {S\&H};
        
            \draw [thick,fill=red!5] ($(sh1.north east)+(0.6,0)$) rectangle node [] (adc1) {\rotatebox{90}{\LARGE ADC}} ($(sh4.south east)+(2.0,0)$);
            \begin{scope}[on background layer]
                \draw (xp11.center) -- (sh1.east) -- +(0.6,0);
                \draw (xp21.center) -- (sh2.east) -- +(0.6,0);
                \draw (xp31.center) -- (sh3.east) -- +(0.6,0);
                \draw (xp41.center) -- (sh4.east) -- +(0.6,0);
            \end{scope}
        \end{scope}
    
        \begin{scope}[shift={(9,0)}]
            \draw (0,0) node [xp] (xp11) {};
            \draw (1,0) node [xp] (xp12) {};
            \draw (2,0) node [xp] (xp13) {};
            \draw (3,0) node [xp] (xp14) {};
            \draw (0,-1) node [xp] (xp21) {};
            \draw (1,-1) node [xp] (xp22) {};
            \draw (2,-1) node [xp] (xp23) {};
            \draw (3,-1) node [xp] (xp24) {};
            \draw (0,-2) node [xp] (xp31) {};
            \draw (1,-2) node [xp] (xp32) {};
            \draw (2,-2) node [xp] (xp33) {};
            \draw (3,-2) node [xp] (xp34) {};
            \draw (0,-3) node [xp] (xp41) {};
            \draw (1,-3) node [xp] (xp42) {};
            \draw (2,-3) node [xp] (xp43) {};
            \draw (3,-3) node [xp] (xp44) {};
            \draw (4,0) node [xp] (xpb1) {};
            \draw (4,-1) node [xp] (xpb2) {};
            \draw (4,-2) node [xp] (xpb3) {};
            \draw (4,-3) node [xp] (xpb4) {};
        
            \draw (5.3,0) node [sh] (sh1) {S\&H};
            \draw (5.3,-1) node [sh] (sh2) {S\&H};
            \draw (5.3,-2) node [sh] (sh3) {S\&H};
            \draw (5.3,-3) node [sh] (sh4) {S\&H};
        
            \draw [thick,fill=red!5] ($(sh1.north east)+(0.6,0)$) rectangle node [] (adc2) {\rotatebox{90}{\LARGE ADC}} ($(sh4.south east)+(2.0,0)$);
            \begin{scope}[on background layer]
                \draw (xp11.center) -- (sh1.east) -- +(0.6,0);
                \draw (xp21.center) -- (sh2.east) -- +(0.6,0);
                \draw (xp31.center) -- (sh3.east) -- +(0.6,0);
                \draw (xp41.center) -- (sh4.east) -- +(0.6,0);
            \end{scope}
        \end{scope}
    
        \draw ($(adc2.east)+(1.5,0)$) node [draw,thick,circle,fill=orange!5,minimum size=2] (sum1) {+};
        \draw[very thick, blue, -stealth] ($(adc2.east)+(0.2,0.0)$) -- (sum1.west);
        \draw[very thick, blue, -stealth] ($(adc1.east)+(0.2,0.0)$) -| +(0.5,2.0) -| (sum1.north);
    \end{scope}

    \begin{scope}[shift={(0,-5)}]
        \begin{scope}[shift={(0,0)}]
            \draw (0,0) node [xp] (xp11) {};
            \draw (1,0) node [xp] (xp12) {};
            \draw (2,0) node [xp] (xp13) {};
            \draw (3,0) node [xp] (xp14) {};
            \draw (0,-1) node [xp] (xp21) {};
            \draw (1,-1) node [xp] (xp22) {};
            \draw (2,-1) node [xp] (xp23) {};
            \draw (3,-1) node [xp] (xp24) {};
            \draw (0,-2) node [xp] (xp31) {};
            \draw (1,-2) node [xp] (xp32) {};
            \draw (2,-2) node [xp] (xp33) {};
            \draw (3,-2) node [xp] (xp34) {};
            \draw (0,-3) node [xp] (xp41) {};
            \draw (1,-3) node [xp] (xp42) {};
            \draw (2,-3) node [xp] (xp43) {};
            \draw (3,-3) node [xp] (xp44) {};
            \draw (4,0) node [xp] (xpb1) {};
            \draw (4,-1) node [xp] (xpb2) {};
            \draw (4,-2) node [xp] (xpb3) {};
            \draw (4,-3) node [xp] (xpb4) {};
        
            \draw (5.3,0) node [sh] (sh1) {S\&H};
            \draw (5.3,-1) node [sh] (sh2) {S\&H};
            \draw (5.3,-2) node [sh] (sh3) {S\&H};
            \draw (5.3,-3) node [sh] (sh4) {S\&H};
        
            \draw [thick,fill=red!5] ($(sh1.north east)+(0.6,0)$) rectangle node [] (adc1) {\rotatebox{90}{\LARGE ADC}} ($(sh4.south east)+(2.0,0)$);
            \begin{scope}[on background layer]
                \draw (xp11.center) -- (sh1.east) -- +(0.6,0);
                \draw (xp21.center) -- (sh2.east) -- +(0.6,0);
                \draw (xp31.center) -- (sh3.east) -- +(0.6,0);
                \draw (xp41.center) -- (sh4.east) -- +(0.6,0);
            \end{scope}
        \end{scope}
    
        \begin{scope}[shift={(9,0)}]
            \draw (0,0) node [xp] (xp11) {};
            \draw (1,0) node [xp] (xp12) {};
            \draw (2,0) node [xp] (xp13) {};
            \draw (3,0) node [xp] (xp14) {};
            \draw (0,-1) node [xp] (xp21) {};
            \draw (1,-1) node [xp] (xp22) {};
            \draw (2,-1) node [xp] (xp23) {};
            \draw (3,-1) node [xp] (xp24) {};
            \draw (0,-2) node [xp] (xp31) {};
            \draw (1,-2) node [xp] (xp32) {};
            \draw (2,-2) node [xp] (xp33) {};
            \draw (3,-2) node [xp] (xp34) {};
            \draw (0,-3) node [xp] (xp41) {};
            \draw (1,-3) node [xp] (xp42) {};
            \draw (2,-3) node [xp] (xp43) {};
            \draw (3,-3) node [xp] (xp44) {};
            \draw (4,0) node [xp] (xpb1) {};
            \draw (4,-1) node [xp] (xpb2) {};
            \draw (4,-2) node [xp] (xpb3) {};
            \draw (4,-3) node [xp] (xpb4) {};
        
            \draw (5.3,0) node [sh] (sh1) {S\&H};
            \draw (5.3,-1) node [sh] (sh2) {S\&H};
            \draw (5.3,-2) node [sh] (sh3) {S\&H};
            \draw (5.3,-3) node [sh] (sh4) {S\&H};
        
            \draw [thick,fill=red!5] ($(sh1.north east)+(0.6,0)$) rectangle node [] (adc2) {\rotatebox{90}{\LARGE ADC}} ($(sh4.south east)+(2.0,0)$);
            \begin{scope}[on background layer]
                \draw (xp11.center) -- (sh1.east) -- +(0.6,0);
                \draw (xp21.center) -- (sh2.east) -- +(0.6,0);
                \draw (xp31.center) -- (sh3.east) -- +(0.6,0);
                \draw (xp41.center) -- (sh4.east) -- +(0.6,0);
            \end{scope}
        \end{scope}
    
        \draw ($(adc2.east)+(1.5,0)$) node [draw,thick,circle,fill=orange!5,minimum size=2] (sum2) {+};
        \draw[very thick, blue, -stealth] ($(adc2.east)+(0.2,0.0)$) -- (sum2.west);
        \draw[very thick, blue, -stealth] ($(adc1.east)+(0.2,0.0)$) -| +(0.5,2.0) -| (sum2.north);
    \end{scope}

    \draw[thick,fill=orange!5] (19,0.5) rectangle node [text width=3.0,align=left,anchor=east] (neu) {\rotatebox{90}{\LARGE Spins \& Annealing}} (20.5,-8.5);
    \draw[very thick, blue, -stealth] (sum1.east) -- +(0.6,0);
    \draw[very thick, blue, -stealth] (sum2.east) -- +(0.6,0);

    \draw[very thick, blue] (20.5,-4) -| +(0.6,-5.5) -| +(-20.5,-5.5) node [] (wlbusleft) {};
    % \begin{scope}[shift={(0,0}]
    \begin{scope}[on background layer]
        \draw[blue] (0,0) |- (wlbusleft);
        \draw[blue] (1,0) |- (wlbusleft);
        \draw[blue] (2,0) |- (wlbusleft);
        \draw[blue] (3,0) |- (wlbusleft);
        \draw[blue] (4,0) |- (wlbusleft);
    \end{scope}
    % \end{scope}
    % \begin{scope}[shift={(9,0}]
    \begin{scope}[on background layer]
        \draw[blue] (9,0) |- (wlbusleft);
        \draw[blue] (10,0) |- (wlbusleft);
        \draw[blue] (11,0) |- (wlbusleft);
        \draw[blue] (12,0) |- (wlbusleft);
        \draw[blue] (13,0) |- (wlbusleft);
    \end{scope}
    % \end{scope}

\end{tikzpicture}

==> fig/naive_tile_floorplan.tikz.tex <==
\begin{tikzpicture}[every node/.style={draw,outer sep=0pt,thick}]
    \node[draw, minimum size=2cm, regular polygon, 
        regular polygon sides=4, 
        label=side 2:$h_{cell}*O_{naive}$, label=side 3:$w_{cell}*I_{naive}$] (PXB) {Primary IMC crossbar};
    \node[draw, right=of PXB, minimum height=2cm, minimum width=1cm, rectangle, label=below:$w_{rblsw}$] (RBLSW) {Output periphery overhead};
    \node[draw, right=of RBLSW, minimum height=2cm, minimum width=1cm, rectangle, label=below:$w_{neuron}$] (sense) {Pipelined ADC};
    \node[draw, right=of sense, circle] (O) {Tile output pins};
    \node[draw, below=of O, circle] (I) {Tile input pins};
    \node[draw, rectangle, below=of PXB, label=left:$h_{rwlsw}$] (RWLSW) {Input periphery overhead};
    \draw [-latex] (PXB) -- (RBLSW);
    \draw [-latex] (RBLSW) -- (sense);
    \draw [-latex] (sense) -- (O);
    \draw [-latex] (sense) |- (RWLSW.north east);
    \draw [-latex] (I.west) |- (RWLSW.south east);
    \draw [-latex] (RWLSW) -- (PXB);
    \draw [thick, label=above:"IMC tile"] ($(PXB.north west)+(-1.6,0.6)$)  rectangle ($(I.south east)+(0.5,-0.6)$);
\end{tikzpicture}
